A Peaceman-Rachford Splitting Approach with Deep Equilibrium Network for Channel Estimation

Multiple-input multiple-output (MIMO) is pivotal for wireless systems, yet its high-dimensional, stochastic channel poses significant challenges for accurate estimation, highlighting the critical need for robust estimation techniques. In this paper, we introduce a novel channel estimation method for the MIMO system. The main idea is to construct a fixed-point equation for channel estimation, which can be implemented into the deep equilibrium (DEQ) model with a fixed network. Specifically, the Peaceman-Rachford (PR) splitting method is applied to the dual form of the regularized minimization problem to construct fixed-point equation with non-expansive property. Then, the fixed-point equation is implemented into the DEQ model with a fixed layer, leveraging its advantage of the low training complexity. Moreover, we provide a rigorous theoretical analysis, demonstrating the convergence and optimality of our approach. Additionally, simulations of hybrid far- and near-field channels demonstrate that our approach yields favorable results, indicating its ability to advance channel estimation in MIMO system.

==> notation.tex <==
\newcommand{\mbbN}{\mathbb{N}} % natural number
\newcommand{\mbbR}{\mathbb{R}} % real number
\newcommand{\mbbC}{\mathbb{C}} % complex number
\newcommand{\mbbP}{\mathbb{P}}
\newcommand{\mbbE}{\mathbb{E}}

\newcommand{\mbfx}{\mathbf{x}} 
\newcommand{\mbfy}{\mathbf{y}} 
\newcommand{\mbfd}{\mathbf{d}} 

\newcommand{\bdW}{\boldsymbol{W}} 
\newcommand{\bdx}{\boldsymbol{x}} 
\newcommand{\bdy}{\boldsymbol{y}} 
\newcommand{\bdz}{\boldsymbol{z}} 
\newcommand{\bdT}{\boldsymbol{T}} 

\newcommand{\bda}{\boldsymbol{\alpha}} 
\newcommand{\bdb}{\boldsymbol{\beta}} 
\newcommand{\bdphi}{\boldsymbol{\phi}} 
\newcommand{\bdpsi}{\boldsymbol{\psi}} 
\newcommand{\bdf}{\boldsymbol{f}} 
\newcommand{\bdg}{\boldsymbol{g}} 
\newcommand{\bdmu}{\boldsymbol{\mu}} 
\newcommand{\bdnu}{\boldsymbol{\nu}} 
\newcommand{\bdp}{\boldsymbol{p}} 
\newcommand{\bdq}{\boldsymbol{q}} 

\newcommand{\mcX}{\mathcal{X}}
\newcommand{\mcY}{\mathcal{Y}}
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcF}{\mathcal{F}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcP}{\mathcal{P}}

\newcommand{\mrmd}{\mathrm{d}}
\newcommand{\mrme}{\mathrm{e}}

\newcommand{\hwu}[1]{{\color{red}#1}}
\newcommand{\stwu}[1]{{\color{blue}#1}}
